Low-Regret Active learning

We develop an online learning algorithm for identifying unlabeled data points that are most informative for training (i.e., active learning). By formulating the active learning problem as the prediction with sleeping experts problem, we provide a regret minimization framework for identifying relevant data with respect to any given definition of informativeness. Motivated by the successes of ensembles in active learning, we define regret with respect to an omnipotent algorithm that has access to an infinity large ensemble. At the core of our work is an efficient algorithm for sleeping experts that is tailored to achieve low regret on easy instances while remaining resilient to adversarial ones. Low regret implies that we can be provably competitive with an ensemble method \emph{without the computational burden of having to train an ensemble}. This stands in contrast to state-of-the-art active learning methods that are overwhelmingly based on greedy selection, and hence cannot ensure good performance across problem instances with high amounts of noise. We present empirical results demonstrating that our method (i) instantiated with an informativeness measure consistently outperforms its greedy counterpart and (ii) reliably outperforms uniform sampling on real-world scenarios.

==> analysis-old.tex <==


Define
$$
\epsilon^* = 
$$
The lemma below shows that $\epsilon^*$ has a very convenient lower bound which will be key in establishing our main theoretical results. 

help establish our claim. In particular, let
$$
\epsilon(x) = \pot[1][x] + \pot[-1][x] - 2\pot[0][0].
$$
Note that $\epsilon(x)$ can be negative.


\begin{lemma}
For all $R \in \Reals, C \in [0, R^2/8]$ and $x \in [-1,1]$,
let 
$$
\epsilon^* = 
$$

and let
$$
\epsilon(x) = \pot[1][x] + \pot[-1][x] - 2\pot[0][0].
$$



$$
\gamma_{R,C}(x) = \frac{\phi_{R,C}(1, x) - \phi_{R,C}(x, x)}{1 - x} - \frac{\phi_{R,C}(x, x) - \phi_{R,C}(-1,x)}{1 + x} \leq \epsilon^* + K
$$
\end{lemma}
\begin{proof}


Now, we seek to maximize $\epsilon(x)$ over $x \in [-1,1]$. Observe that $\epsilon(x)$ is convex with respect to $x \in [-1,1]$ since its second derivative is non-negative under the conditions of the lemma. This implies that $\epsilon(x)$ takes its maximum value at a boundary point, i.e., either at $x=-1$ or $x=1$. To distinguish the optimal point, consider more formally the derivative of $\epsilon(x)$ with respect to $x$
$$
\epsilon'(x) = \frac{(a+1)^2}{4(a+b-x+2)^2} \pot[1][x] - \frac{(a-1)^2}{4 (a+b+x)^2} \pot[-1][x].
$$
Note that since $\epsilon(x)$ is convex, its derivative is minimized at the left boundary $x=-1$. This means that if we can show that $\epsilon'(-1) \ge 0$, then this would imply that $\epsilon(x)$ is increasing for all $x \in [-1,1]$ and hence maximized at $\epsilon(1)$, which is the statement of the lemma.

Consider 
$$
\epsilon'(-1) = \frac{(a+1)^2}{4(a+b+3)^2} \pot[1][-1] - \frac{(a-1)^2}{4 (a+b-1)^2} \pot[-1][-1].
$$

To show that $\epsilon'(-1) \ge 0$, we will show the following ratio between the two expressions above, defined by $\rho(a,b)$, is at least 1:
\begin{align*}
\rho(a, b) &= \frac{(a+1)^2}{4(a+b+3)^2} \pot[1][-1] \left (\frac{(a-1)^2}{4 (a+b-1)^2} \pot[-1][-1] \right)^{-1} \\
&= \frac{(1+a)^2 (a + b -1)^2}{(a-1)^2(a + b + 3)^2} \exp \left(\frac{a + ab -1}{(a + b -1)(a+b+3)} \right).
\end{align*}
Taking the derivative of $\rho(a,b)$ with respect to $b$, we obtain that the derivative is positive for $b < b^*$ and negative for $b > b^*$ for some $b^*$. This implies that $b^*$ is a local maximum, and so the minimum $\min_{b \ge 4} \rho(a,b)$ occurs at either boundary $b = 4$ or as $b \to \infty$. For $b = 4$, we obtain
\begin{align*}
    \rho(a,4) &= \left(  \frac{(1+a) (3+a)}{(a-1)(7+a)}\right)^2 \exp \left(\frac{9}{7+a} - \frac{4}{3+a} \right) \\
    &\ge \lim_{a \to \infty} \rho(a, 4) \\
    &= 1
\end{align*}
(Note that we would've had $\rho(a,b) < 1$ if we allowed for $b < 4$. $b$ has to be 4 here!).
where the inequality follows from the fact that $\rho(a,4)$ is monotonically decreasing for $a > 1$.
On the other hand, we also have
\begin{align*}
    \lim_{b->\infty} \rho(a,b) &= 1 + \frac{4a}{(a-1)^2} \\
        &\ge 1 + \min_{a \ge 2} \frac{4a}{(a-1)^2} \\
        &= 1.
\end{align*}
Thus, we've shown that $\rho(a,b) \ge 1$, which implies that $\epsilon'(-1) \ge 0$ and this shows that $\epsilon(x) \leq \epsilon(1)$.


 Taking the derivative of $\epsilon(x)$, we find that 

Applying Lemma 2 of ~\cite{luo2014drifting} (also see end of the proof of Lemma 5 in~\cite{luo2015achieving}), we obtain
$$
\epsilon(x) \leq \epsilon^*.
$$

Assume for the sake of contradiction that $\gamma_{R,C}(x) > \eps^*$, then
\begin{align*}
    \pot[1][x] - &\pot[-1][x] \\
    &= \pot[1][x] - \pot[x][x] + \pot[x][x] - \pot[-1][x] \\
    &= (1 - x) \frac{\pot[1][x] - \pot[x][x]}{1-x} + (1 + x) \frac{\pot[x][x] - \pot[-1][x]}{1+x} \\
    &< (1 - x) \frac{\pot[1][x] - \pot[x][x]}{1-x} + (1+x) \left(\frac{\pot[1][x] - \pot[x][x]}{1-x} - \eps^* \right) \\
    &= 2 \left(\frac{\alpha_{R,C}(1) - \beta_{R,C}(x)}{1-x} \right) - (1+x) \eps^*.
\end{align*}
This also implies that
$$
\pot[1][x] - \pot[-1][x] \leq 2 \gamma(x).
$$
Note that since $\epsilon^* \ge 0$, for $x \in [0,1]$, we have $$(1+x) \epsilon^* \ge \epsilon^* \ge \epsilon(x) \Rightarrow -(1+x) \epsilon^* \leq -\epsilon(x).$$ Combining this with the inequality from above implies that, if $\gamma_{R,C}(x) > \eps^*$, then
\begin{equation}
    \label{eqn:pos-case}
    \forall{x \in [0,1]} \quad 
    \pot[1][x] - \pot[-1][x] < 2 \left(\frac{\alpha_{R,C}(1) - \beta_{R,C}(x)}{1-x} \right) - \epsilon(x).
\end{equation}
Now we would also like to have an inequality for $ x\in [-1,0]$. To obtain one, note that we also have
\begin{align*}
    \pot[1][x] - \pot[-1][x] &> (1-x) \left( \frac{\beta(x) - \beta(-1)}{1+x} + \eps^* \right) + (1+x) \left(\frac{\beta(x) - \beta(-1)}{1+x} \right)\\
    &= 2 \left(\frac{\beta(x) - \beta(-1)}{1 + x}  \right) + (1-x)\eps^*.
\end{align*}
Similar to the reasoning above: since $\epsilon^* \ge 0$, for $x \in [-1,0]$ observe that
$$
(1-x) \eps^* \ge \eps^* \ge \eps(x).
$$
Hence, we obtain the condition that, if  $\gamma_{R,C}(x) > \eps^*$, then we must have
\begin{equation}
    \label{eqn:neg-case} 
    \forall{x \in [0,1]} \quad 
     \pot[1][x] - \pot[-1][x] > 2 \left(\frac{\beta(x) - \beta(-1)}{1 + x}  \right) + \eps(x).
\end{equation}

Having established the implications \eqref{eqn:pos-case} and \eqref{eqn:neg-case} resulting from the assumption $\gamma_{R,C}(x) > \eps^*$, we proceed via a proof by contrapositive. In other words, we will show via a case-by-case proof that if $x \in [0,1]$, then the inequality in \eqref{eqn:pos-case} is false, and if $x \in [-1,0)$, then the inequality in \eqref{eqn:neg-case} is false, which will establish the claim that $\gamma_{R,C}(x) \leq \eps^*$.


\subsection{Case $x > 0$}
In this case, we would like to arrive at a contradiction by showing that \eqref{eqn:pos-case} is false, i.e., we want to show
$$
\pot[1][x] - \pot[-1][x] \ge 2 \left(\frac{\alpha_{R,C}(1) - \beta_{R,C}(x)}{1-x} \right) - \eps(x)
$$
Plugging in the definition of $\eps(x)$, we see that this is equivalent to
$$
\pot[1][x] - \pot[0][0] \ge \frac{\alpha_{R,C}(1) - \beta_{R,C}(x)}{1-x}.
$$
Rearranging, we see that we must show that
$$
\underbrace{\beta_{R,C}(x) - \pot[0][0] - x (\pot[1][x] - \pot[0][0])}_{\text{concave with respect to x} \in [0,1]} \ge 0,
$$
where the claim about concavity follows from evaluation of the second derivative, which is non-positive for all $x \in [0,1]$ under the assumption that $b \leq a^2/8$. We see that the inequality above indeed holds by Bauer's minimum principle, i.e., the function above is continuous and concave on a convex and compact set $[0,1]$, and so it attains its minimum values at an extreme point, i.e., either $0$ or $1$, both at which the function above yields 0. This completes the case $x \geq 0$.


\subsection{Case $x < 0$}
Mirroring the case prior, we will show that \eqref{eqn:neg-case} is false, i.e., we would like to prove that
$$
    \pot[1][x] - \pot[-1][x] \leq  2 \left(\frac{\beta(x) - \beta(-1)}{1 + x}  \right) + \eps(x).
$$
Plugging in $\epsilon(x) = \pot[1][x] + \pot[-1][x] - 2\pot[0][0]$ and rearranging yields
$$
\pot[0][0] - \pot[x][x] + x(\pot[0][0] - \pot[-1][x]) \leq 0.
$$


For a fixed $r' \in [-1,1]$ and $x \in [-1,1]$ define two convex functions
$$
\alpha_{R,C}(x) = \exp \left ( \frac{(a+x)^2}{a + b + 2x - r'} \right)
$$
and
$$
\beta_{R,C}(x) = \exp \left ( \frac{(a+x)^2}{a + b + r'} \right).
$$
By definition, we have $\alpha_{R,C}(1) = \pot[1][r']$, $\alpha_{R,C}(r') = \beta_{R,C}(r') = \pot[r'][r']$, and $\beta_{R,C}(-1) = \pot[-1][r']$. Thus,
$$
\gamma_{R,C}(x) = \frac{\alpha_{R,C}(1) - \alpha_{R,C}(r')}{1- x} - \frac{\beta_{R,C}(r') - \beta_{R,C}(-1)}{1 + r'}.
$$

% Now note that
% \begin{align*}
%     &\alpha'_{R,C}(x) = \left (\frac{2 (a+x) (b+ x - r')}{3 (a+b+2x - r')^2} \right) \alpha_{R,C}(x), \quad \text{and} \\
%     &\alpha''_{R,C}(x) = \left( \frac{(4 (a + x)^2 (b + x - r')^2}{(9 (a + b + 2 x - r')^4)} + \frac{2 (a - b + r')^2}{3 (a + b + 2 x - r')^3} \right) \alpha_{R,C}(x).
% \end{align*}


% Applying Taylor's Theorem to $\alpha_{R,C}(1)$ around $r'$, we have
% \begin{align*}
% \alpha_{R,C}(1) &= \alpha_{R,C}(r') + (1 - r') \alpha'_{R,C}(r') + \frac{(1 - r')^2 \alpha''_{R,C}(\xi)}{2} \\
% &\leq 
% \end{align*}

\end{proof}


==> analysis_new.tex <==


\begin{lemma}[Greedy incurs linear regret]

\end{lemma}
\begin{proof}
WLOG, consider the setting with $n = 3$ points and oblivious losses at each round defined by a simple coin flip:

\begin{align*}
\ell_t =       \begin{cases} (\epsilon, 0, 1)  \text{ with probability $1/2$}, \\
         (\epsilon, 1, 0) \text{ with probability $1/2$}
        \end{cases}
\end{align*}
where $\varepsilon \in (0, 1/2)$. 

This means that for any *realization* of $\ell_t$, the optimal point is either the second or third one according to greedy. Hence, greedy would either pick the second or third data point (whichever has 0 loss) at each time step. But, if we consider the *expected loss vector* over the randomness in the training (which is what we care about in regret $\mathcal R$), we have for all $t$

$$\mathbb E_{\xi_{t-1}}[\ell_t(\theta_{t-1}) | \mathcal F_{t-1}] = (\epsilon, 1/2, 1/2) \quad \forall{\mathcal F_{t-1}}.$$

This implies that in fact the first point is optimal (since $\varepsilon \in (0,1/2)$) with respect to our definition of robustness (expected loss over the randomness in training). 

This means that greedy leads to an expected regret of $\mathbb E [\mathcal R(\xi_{0:T-1}, \mathcal S_{1:T})] = T (1/2 - \varepsilon)$, which is linear in $T$. 

In contrast to greedy, our approach obtains the expected regret (as derived in our last response): 

$\mathbb E [\mathcal R(\xi_{0:T-1}, \mathcal S_{1:T})] \leq \mathcal O (\sqrt{T})$

(since the optimal distribution doesn’t change, $V(u^*) = 1$)

This is also obtained by taking the expectation of both sides of the bound in our initial response.

This counterexample additionally proves the suboptimality of the greedy variant that you recommended which considers the loss at $\theta_{t-2}$ instead of $\theta_{t-1}$. This is because the greedy variant will still pick either the second or third point given that it only has access to the realization of the loss at $\theta_{t-2}$ -- either $(\varepsilon, 0, 1)$ or $(\varepsilon, 1, 0)$ --  at each time step.
\end{proof}






\section{Analysis of Expected Regret}
For sake of simplicity, consider active learning with a batch size of $1$, i.e., $|\mathcal S_1| = \cdots = |\mathcal S_T| = 1$ — the generalization follows by linearity of expectation. Let $\ell_{t \, \mathcal S_t}(\cdot)$ denote the loss corresponding to $\mathcal S_t \sim p_t$ at iteration $t$ and let $\mathcal F_t = \sigma(\xi_0, \mathcal S_1, \ldots, \xi_{t-1}, \mathcal S_t)$ be the filtration. We will abbreviate the loss of selected point $\mathcal S_t$ as $\ell_{t \mathcal S_t}$ with the understanding that it additionally depends on the random variables $\mathcal S_{1:t-1}$ and $\xi_{0:t-1}$. Our goal is to bound the regret of the sampled point $\mathcal S_t$ over the randomness in the \emph{network noise} $\xi_{t-1}$ conditioned on our past actions and observations (i.e., filtration $\mathcal F_{t-1}$). 

For any sequence of realizations $\xi_{0:T-1}$ and $\mathcal S_{1:T}$, define our realized regret wrt the optimal sequence of distributions $u_1^*, \ldots, u_t^*$ as 


$
\mathcal R (\xi_{0:T-1}, \mathcal S_{1:t-1}) = \sum_{t=1}^T \mathbb E_{\xi_{t-1}, \mathcal S_t} [\ell_{t \mathcal S_t} | \mathcal F_{t-1}] - \mathbb E_{\xi_{t-1}} [\langle u_t^*, \ell_{t} \rangle | \mathcal F_{t-1}].
$

(To be clear, $\ell_{t} = \ell_t \left(\mathcal M(\cup_{\tau = 1}^{t-1} \mathcal S_\tau, \xi_{t-1})\right)$ in the above, which is why we take the expectation over $\xi_{t-1}$)

Note that $\mathcal R$ is a random variable over $\xi_{0:T-1}$ and $\mathcal S_{1:T}$ due to the conditioning.


By the fact that $\mathcal S_t \sim p_t$ we have

$
\mathbb E_{\mathcal S_t} [ \ell_{t \mathcal S_t} | \mathcal F_{t-1}, \xi_{t-1}] = \langle p_t,\ell_t \rangle.
$

Applying this in conjunction with the tower property for conditional expectation ($\mathbb E [V | W] = \mathbb E [ \mathbb E [V| U, W] | W]$) yields

$
\mathbb E_{\xi_{t-1}, \mathcal S_t} [ \ell_{t \mathcal S_t} | \mathcal F_{t-1}] = \mathbb E_{\xi_{t-1}} [ \mathbb E_{\mathcal S_t} [ \ell_{t \mathcal S_t} | \mathcal F_{t-1}, \xi_{t-1}] | \mathcal F_{t-1}] = \mathbb E_{\xi_{t-1}} [ \langle p_t,\ell_t \rangle| \mathcal F_{t-1}].
$


Taking the expectation over all the randomness up to time step $t$ of the above leads to

$
\mathbb E_{\xi_{0:t-2}, \mathcal S_{1:t-1}}[ \mathbb E_{\xi_{t-1}, \mathcal S_t} [ \ell_{t \mathcal S_t} | \mathcal F_{t-1}] ] = \mathbb E_{\xi_{0:t-2}, \mathcal S_{1:t-1}}[ \mathbb E_{\xi_{t-1}} [ \langle p_t,\ell_t \rangle|\mathcal F_{t-1}] ] = \mathbb E_{\xi_{0:t-1}, \mathcal S_{1:t-1}}[\langle p_t,\ell_t \rangle],
$

where the last equality is by the towering property. Hence, we obtain for the expected regret:

$
\mathbb E_{\xi_{0:T-1}, \mathcal S_{1:T}} [ \mathcal R (\xi_{0:T-1}, \mathcal S_{1:t-1})] = \sum_{t=1}^T  \mathbb E_{\xi_{0:t-1}, \mathcal S_{1:t-1}} [ \langle p_t - u_t^*, \ell_t\rangle ] = \mathbb E_{\xi_{0:T-1}, \mathcal S_{1:T-1}} [\sum_{t=1}^T  \langle p_t - u_t^*,\ell_t\rangle ].
$

And so applying Theorem 2, which works for any sequence of losses gives us a bound on the expected regret:
$
\mathbb E_{\xi_{0:T-1}, \mathcal S_{1:T}} [ \mathcal R (\xi_{0:T-1}, \mathcal S_{1:t-1})] \leq \mathbb E_{\xi_{0:T-1}, \mathcal S_{1:T}} \mathcal{O} \left( \sqrt{\big(1 + \displaystyle \sum \nolimits_{t } ||\ell_{t}(\theta_{t-1}) - \ell_{t-1}(\theta_{t-2})||_\infty^2 \big) \mathcal{V}(u^*)} \right ).
$

The generalization to the sleeping experts setting follows by noting that the set of awake experts at iteration $t$, i.e.,  $\mathcal I_t$, is $\mathcal F_{t-1}$-measurable (since it just depends on which points we have picked thus far), so by the same logic as above, we obtain the upper bound on the sleeping experts regret of

$
\mathbb E_{\xi_{0:T-1}, \mathcal S_{1:T}} \mathcal{O} \left( \sqrt{\big(1 + \displaystyle \sum \nolimits_{t } ||(\ell_{t}(\theta_{t-1}) - \ell_{t-1}(\theta_{t-2})) \odot \mathcal I_{t} ||_\infty^2 \big) \mathcal{V}(u^*)} \right ).
$


==> pseudocode-al-regret.tex <==
\begin{algorithm}
\small
\caption{\textsc{ActiveLearning}}
\label{alg:active-learning}
\textbf{Input:} Set of points $\PP \subseteq \Reals^{d \times n}$, \textsc{Acquire:} an active learning algorithm for selecting labeled points
\begin{spacing}{1}
\begin{algorithmic}[1]
\small

\STATE $\SS \gets \emptyset$; \, $\theta_0 \gets \text{Randomly initialized network model}$;
\FOR{$t \in [T]=\{1, \ldots, T\}$} %\label{lin:start-active}
    \STATE $\SS_t \gets \textsc{Acquire}(\PP \setminus \SS, b_t, \theta_{t-1})$ \COMMENT{Get new batch of $b_t \in \mathbb{N}_+$ points to label using algorithm \textsc{Acquire}} \\
    \STATE $\SS \gets \SS \cup \SS_t$ \COMMENT{Add new  points} \\
    \STATE (if \textsc{Scratch} option) $\theta_{t-1} \gets \text{Randomly initialized network}$
    \STATE $\theta_t \gets \textsc{Train}(\theta_{t-1}, \{\left(x, \textsc{Oracle}(x)\right)_{x \in \SS} \})$ \COMMENT{Train network on the labeled samples thus far} \\ 
    % \STATE $\textsc{AdaHedge.SufferLoss}(w_t, p_t)$ \COMMENT{Update AdaHedge based on the current "loss" with respect to prediction $p_t$ and network state $w_t$, i.e., this is the "incur loss" step in traditional online learning} 

\ENDFOR %\label{lin:end-active}
\STATE \textbf{return} $\theta_T$

\end{algorithmic}
\end{spacing}
\end{algorithm}
